Comparison of Static Analysis Architecture Recovery Tools for Microservice Applications

Architecture recovery tools help software engineers obtain an overview of the structure of their software systems during all phases of the software development life cycle. This is especially important for microservice applications because they consist of multiple interacting microservices, which makes it more challenging to oversee the architecture. Various tools and techniques for architecture recovery (also called architecture reconstruction) have been presented in academic and gray literature sources, but no overview and comparison of their accuracy exists. This paper presents the results of a multivocal literature review with the goal of identifying architecture recovery tools for microservice applications and a comparison of the identified tools' architectural recovery accuracy. We focused on static tools since they can be integrated into fast-paced CI/CD pipelines. 13 such tools were identified from the literature and nine of them could be executed and compared on their capability of detecting different system characteristics. The best-performing tool exhibited an overall F1-score of 0.86. Additionally, the possibility of combining multiple tools to increase the recovery correctness was investigated, yielding a combination of four individual tools that achieves an F1-score of 0.91. Registered report: The methodology of this study has been peer-reviewed and accepted as a registered report at MSR'24: arXiv:2403.06941

==> 42_Dataset_extension.tex <==
\section{Extended Dataset}
\label{sec:extended_dataset}

Based on the selection of tools that could be part of the comparison and the tool characterization matrix (Table~\ref{tbl:characteristics_matrix}), the dataset needed to be extended with only a single characteristic, endpoints.
Although such information was already contained in the dataset, it was not exhaustive and could not serve as ground truth for the comparison in that state.

The dataset was thus extended following the methodology presented in Section~\ref{sec:methodology}, i.e., by manually identifying all instances of Java's \texttt{RequestMapping} annotation and related more specific annotations (\texttt{PostMapping}, \texttt{DeleteMapping}, and more) and all instances of the \texttt{@RepositoryRestResource} annotation in the dataset's applications.
We identified 63 additional endpoints following this process.
As a result, the extended dataset now contains exhaustive information about endpoints specified with the considered Java annotations.

Since some of this paper's authors are also authors of the initial dataset, we have integrated the described changes directly.
All means of obtaining the dataset have been updated to the new data (the corresponding website~\footnote{https://tuhh-softsec.github.io/microSecEnD/} and GitHub repository~\footnote{https://github.com/tuhh-softsec/microSecEnD} contain the new data, and we added a new version containing the new data to the persistent repository at Zenodo~\footnote{https://zenodo.org/records/7714926}).



